DeepCaps: Going Deeper with Capsule Networks

Capsule Network is a promising concept in deep learning, yet its true potential is not fully realized thus far, providing sub-par performance on several key benchmark datasets with complex data. Drawing intuition from the success achieved by Convolutional Neural Networks (CNNs) by going deeper, we introduce DeepCaps1, a deep capsule network architecture which uses a novel 3D convolution based dynamic routing algorithm. With DeepCaps, we surpass the state-of-the-art results in the capsule network domain on CIFAR10, SVHN and Fashion MNIST, while achieving a 68% reduction in the number of parameters. Further, we propose a class-independent decoder network, which strengthens the use of reconstruction loss as a regularization term. This leads to an interesting property of the decoder, which allows us to identify and control the physical attributes of the images represented by the instantiation parameters.

==> methods_deep_caps_skip.tex <==
% %!TEX root = ../egpaper_for_review.tex
% \subsection{DeepCaps+Skip}
% Reconstructed images from the capsule model\cite{sabour2017dynamic} and our DeepCaps model are blurry and lacks sufficient low level information such as edges and lines. Even though the primary reason for this unsatisfactory performance is that the 16 dimensional capsule vector cannot represent a sufficient amount of the lower-level information in the image and the conspicuous solution is to increase the dimensionality of the capsule vector, it is not a feasible solution in an attempt in going deeper, as any increase the capsule vector dimentionality will exponentially increase the cost of routing and memory. Therefore, we propose to use skip connections between \texttt{ConvCaps} layer in the DeepCaps Network and the corresponding Deconvolutional layer in the decoder network. We hypothesize that the addition of the skip connections will not only improve the reconstructions, yet also by allowing the gradients to back propagate from decoder network to the capsule filters will aid them to learn better understanding of the image. Simultaneously, this will ease the burden of capturing all the information in the image, from the DeepCaps network, such that it can focus only on learning high level information from the image, while the skip connections take care of the low level information.

% \subsubsection{DeepCaps+BG+Skip}
% As shown in the results section 5.1, we combine both background capsule and skip connection to our model. We hypothesize that the combination of background capsules and skip connection between capsule and decoder network will outperform the individual variations proposed in sections 3.11 and 3.12. 
